Weak-shot Semantic Segmentation via Dual Similarity Transfer

Semantic segmentation is an important and prevalent task, but severely suffers from the high cost of pixel-level annotations when extending to more classes in wider applications. To this end, we focus on the problem named weak-shot semantic segmentation, where the novel classes are learnt from cheaper image-level labels with the support of base classes having off-the-shelf pixel-level labels. To tackle this problem, we propose SimFormer, which performs dual similarity transfer upon MaskFormer. Specifically, MaskFormer disentangles the semantic segmentation task into two sub-tasks: proposal classification and proposal segmentation for each proposal. Proposal segmentation allows proposal-pixel similarity transfer from base classes to novel classes, which enables the mask learning of novel classes. We also learn pixel-pixel similarity from base classes and distill such class-agnostic semantic similarity to the semantic masks of novel classes, which regularizes the segmentation model with pixel-level semantic relationship across images. In addition, we propose a complementary loss to facilitate the learning of novel classes. Comprehensive experiments on the challenging COCO-Stuff-10K and ADE20K datasets demonstrate the effectiveness of our method. Codes are available at https://github.com/bcmi/SimFormer-Weak-Shot-Semantic-Segmentation.

==> fig_blocks/fig1.tex <==
\begin{figure}[t]
\begin{minipage}[t]{0.47\linewidth}
\centering
\includegraphics[width=1\textwidth]{fig_imgs/setting_overview.jpg}
\caption{  
Illustration for the motivation of our learning scenario.
Off-the-shelf semantic datasets focus on certain base classes, \emph{i.e.}, the colored masks in subfigure (b), while left the novel classes as ignored, \emph{i.e.}, the regions in black.
We would like to segment novel classes by virtue of cheaper image-level labels, instead of annotating expensive pixel-level masks.
}
\label{fig:setting_overview}
\end{minipage}\quad \quad
\begin{minipage}[t]{0.47\linewidth}  
\includegraphics[width=1\textwidth]{fig_imgs/method_overview.jpg}
\caption{  
Overview of our proposed framework.
We use MaskFormer \cite{MaskFormer} to obtain proposal embedding and pixel embeddings for each image.
The transferred proposal-pixel similarity could produce mask for proposal embeddings of novel classes, while the transferred pixel-pixel similarity could help to produce more detailed mask.
Best view in colors.
}
\label{fig:method_overview}
\end{minipage}
% \vspace{-15pt}
\end{figure}

